Geometric Adversarial Attacks and Defenses on 3D Point Clouds

Deep neural networks are prone to adversarial examples that maliciously alter the network's outcome. Due to the increasing popularity of 3D sensors in safety-critical systems and the vast deployment of deep learning models for 3D point sets, there is a growing interest in adversarial attacks and defenses for such models. So far, the research has focused on the semantic level, namely, deep point cloud classifiers. However, point clouds are also widely used in a geometric-related form that includes encoding and reconstructing the geometry. In this work, we are the first to consider the problem of adversarial examples at a geometric level. In this setting, the question is how to craft a small change to a clean source point cloud that leads, after passing through an autoencoder model, to the reconstruction of a different target shape. Our attack is in sharp contrast to existing semantic attacks on 3D point clouds. While such works aim to modify the predicted label by a classifier, we alter the entire reconstructed geometry. Additionally, we demonstrate the robustness of our attack in the case of defense, where we show that remnant characteristics of the target shape are still present at the output after applying the defense to the adversarial input. Our code is publicly available at https://github.com/itailang/geometric_adv.

==> figures/attack/attack_png.tex <==
\begin{figure*}[tb!]
\begin{center}
\begin{tabular}{ c c c c c }
Clean  & Latent space  & Output space  & \new{Semantic} & Clean \\
source & attack (ours) & attack (ours) & \new{attack~\cite{xiang2019generating}} & target \\

\includegraphics[width=0.14\linewidth]{figures/attack/src_table_19_target_sofa_3_input.png} &
\includegraphics[width=0.14\linewidth]{figures/attack/latent_space/latent_os.png} &
\includegraphics[width=0.14\linewidth]{figures/attack/output_space/output_os.png} &
\includegraphics[width=0.14\linewidth]{figures/attack/semantic_attack/semantic_os.png} &
\includegraphics[width=0.14\linewidth]{figures/attack/tgt_table_19_target_sofa_3_input.png} \\

\includegraphics[width=0.14\linewidth]{figures/attack/src_table_19_target_sofa_3_recon.png} &
\includegraphics[width=0.14\linewidth]{figures/attack/latent_space/adv_table_19_target_sofa_3_recon.png} &
\includegraphics[width=0.14\linewidth]{figures/attack/output_space/adv_table_19_target_sofa_3_recon.png} &
\includegraphics[width=0.14\linewidth]{figures/attack/semantic_attack/adv_table_19_target_sofa_recon.png} &
\includegraphics[width=0.14\linewidth]{figures/attack/tgt_table_19_target_sofa_3_recon.png} \\

N/A & $\TNRE = 1.03$ & $\TNRE = 0.85$ & N/A & $\TNRE = 1.00$ \\

\end{tabular}
\caption{{\bfseries \new{Attacks comparison}.} Top row: a clean source point cloud (\textit{table}), adversarial examples of the latent and output space attacks, \new{a semantic adversarial example (targeted to the label \textit{sofa}),} and a clean target (\textit{sofa}). Bottom row: corresponding reconstructions and their target normalized reconstruction error, $\TNRE$ (not applicable for the reconstructed source \new{and the semantic attack}). We mark off-surface ($OS$) points for the attacks with arrows (part of them, to avoid clutter). \new{Both our attacks alter the reconstructed geometry to the desired target shape, while the output space attack results in a smaller perturbation of the input point set compared to the latent space attack. In contrast, the semantic adversarial example fails to attack the autoencoder and is \textit{not} reconstructed as a sofa, but rather as a table.}}
\label{fig:attack}
\end{center} 
\end{figure*}

%\new{The semantic adversarial example fails to attack the autoencoder and is \textit{not} reconstructed as a sofa, but rather as a table. In contrast, both our attacks alter the reconstructed geometry to the desired target shape, while the output space attack results in a smaller perturbation of the input point set compared to the latent space attack.}

%In contrast, both our attacks matches the AE’s reconstruction quality for a clean target, while the output space attack results in a smaller perturbation of the input point set compared to the latent space attack.

%Top row: a clean source point cloud (\textit{table}), adversarial examples of latent and output space attacks, and a clean target (\textit{sofa}). Bottom row: corresponding reconstructions and their target normalized reconstruction error, $\TNRE$. We mark off-surface ($OS$) points for the attacks with arrows (only part of them to avoid clutter). The output space attack usually results in less distortion of the source shape than the latent space attack and matches the AE's reconstruction quality for a clean target.

==> figures/attack_tradeoff/tradeoff_png.tex <==
\begin{figure}[tb!]
\begin{center}
\begin{tabular}{ c c c }
Output space  & Output space & Output space  \\
attack ($\lambda = 10$) & attack ($\lambda = 20$) & attack ($\lambda = 30$) \\

\includegraphics[width=0.28\linewidth]{figures/attack_tradeoff/lambda_10/adv_bench_21_target_car_1_input.png} &
\includegraphics[width=0.28\linewidth]{figures/attack_tradeoff/lambda_20/adv_bench_21_target_car_1_input.png} &
\includegraphics[width=0.28\linewidth]{figures/attack_tradeoff/lambda_30/adv_bench_21_target_car_1_input.png} \\

\includegraphics[width=0.28\linewidth]{figures/attack_tradeoff/lambda_10/adv_bench_21_target_car_1_recon.png} &
\includegraphics[width=0.28\linewidth]{figures/attack_tradeoff/lambda_20/adv_bench_21_target_car_1_recon.png} &
\includegraphics[width=0.28\linewidth]{figures/attack_tradeoff/lambda_30/adv_bench_21_target_car_1_recon.png} \\

Reconstructed     & Reconstructed     & Reconstructed     \\
adversarial input & adversarial input & adversarial input \\
\end{tabular}
\caption{{\bfseries Attack trade-off.} Top row: . Bottom row: .}
\label{fig:supp_attack_tradeoff}
\end{center}
\end{figure}


==> figures/defense/defense_png.tex <==
\begin{figure*}[tb!]
\begin{center}
\begin{tabular}{ c c c c }
Clean  & Output space & Off-surface & Critical points \\
source & attack       & defense        & defense         \\

\includegraphics[width=0.14\linewidth]{figures/defense/src_table_17_target_sofa_4_input.png} &
\includegraphics[width=0.14\linewidth]{figures/defense/adv_table_17_target_sofa_4_input.png} &
\includegraphics[width=0.14\linewidth]{figures/defense/surface/def_table_17_target_sofa_4_input.png} &
\includegraphics[width=0.14\linewidth]{figures/defense/critical/def_table_17_target_sofa_4_input.png} \\

\includegraphics[width=0.14\linewidth]{figures/defense/src_table_17_target_sofa_4_recon.png} &
\includegraphics[width=0.14\linewidth]{figures/defense/adv_table_17_target_sofa_4_recon.png} &
\includegraphics[width=0.14\linewidth]{figures/defense/surface/def_table_17_target_sofa_4_recon.png} &
\includegraphics[width=0.14\linewidth]{figures/defense/critical/def_table_17_target_sofa_4_recon.png} \\

$\SNRE = 1.00$ & $\SNRE = 10.75$    & $\SNRE = 2.96$ & $\SNRE = 2.82$ \\

\end{tabular}
\caption{{\bfseries Off-surface and critical points defenses.} Top row: a clean source point cloud (\textit{table}), an adversarial example of the output space attack (targeted to a \textit{sofa}), defended point cloud by the off-surface defense, and defended point cloud by the critical points defense. Bottom row: corresponding reconstructions and their source normalized reconstruction error, $\SNRE$, before defense (two results on the left) and after defense (two results on the right). While both defenses remove offensive points from the input, remnants of the attack's target still appear in the output reconstruction. Here, instead of a flat surface, the top of the reconstructed table after defense resembles the sofa's seat.}
\label{fig:defense}
\end{center}
\end{figure*}

%Top row: a clean source point cloud (\textit{table}), an adversarial example of the output space attack (targeted to a \textit{sofa}), and defended point clouds by off-surface and critical points defenses. Bottom row: corresponding reconstructions. While both defenses remove offensive points from the input, remnants of the attack's target still appear in the output reconstruction. In this example, instead of a flat surface, the top of the reconstructed table after defense resembles the sofa's seat.


==> figures/target/target_pdf.tex <==
\begin{figure}[tb!]
\begin{center}
\includegraphics[width=\columnwidth]{figures/target/target.pdf}
\caption{{\bfseries Target selection.} For a given source point cloud in shape class $\EuScript{S}$, we select its geometric nearest neighbors, in the sense of Chamfer Distance, from a target shape class $\EuScript{T}$. These point clouds serve as candidates for the attack's target. Here, we illustrate the geometrically closest target \textit{car} instance $T$ for a source \textit{bench} shape $S$.}
\label{fig:target_selection}
\end{center}
\end{figure}

==> figures/teaser/teaser_png.tex <==
\begin{figure}[t!]
\begin{center}
\begin{tabular}{ c c c }
Clean  & Semantic & Geometric     \\
source & attack   & attack (ours) \\

\includegraphics[width=0.28\linewidth]{figures/teaser/output_attack/src_bench_21_target_car_1_input.png} &
\includegraphics[width=0.28\linewidth]{figures/teaser/semantic_attack/adv_bench_21_target_car_input.png} &
\includegraphics[width=0.28\linewidth]{figures/teaser/output_attack/adv_bench_21_target_car_1_input.png} \\

\includegraphics[width=0.28\linewidth]{figures/teaser/output_attack/src_bench_21_target_car_1_recon.png} &
\includegraphics[width=0.28\linewidth]{figures/teaser/semantic_attack/adv_bench_21_target_car_recon.png} &
\includegraphics[width=0.28\linewidth]{figures/teaser/output_attack/adv_bench_21_target_car_1_recon.png} \\
\end{tabular}
\caption{{\bfseries A geometric adversarial attack.} Given a clean input point cloud (top left), our attack crafts an adversarial example (top right) that changes the \textit{geometry} at the output of an \textit{autoencoder} model (bottom row). In this example, it turns a \textit{bench} into a \textit{car}.}
\label{fig:teaser}
\end{center}
\end{figure}

%Our attack crafts an adversarial example (top right) from a clean input point cloud (top left), in order to change the \textit{geometry} at the output of an autoencoder (bottom row). In this example, it turns a \textit{bench} into a \textit{car}.

%Top row: Clean input and adversarial input.  Bottom rows: reconstructed point cloud the corresponding input. Our attack generates a moderate perturbation to the input, while dramatically changing the geometry of the output. In this example, it turns a \textit{bench} into a \textit{car}.
